Multiple Interactions Made Easy (MIME): Large Scale Demonstrations Data for Imitation

In recent years, we have seen an emergence of data-driven approaches in robotics. However, most existing efforts and datasets are either in simulation or focus on a single task in isolation such as grasping, pushing or poking. In order to make progress and capture the space of manipulation, we would need to collect a large-scale dataset of diverse tasks such as pouring, opening bottles, stacking objects etc. But how does one collect such a dataset? In this paper, we present the largest available robotic-demonstration dataset (MIME) that contains 8260 human-robot demonstrations over 20 different robotic tasks (https://sites.google.com/view/mimedataset). These tasks range from the simple task of pushing objects to the difficult task of stacking household objects. Our dataset consists of videos of human demonstrations and kinesthetic trajectories of robot demonstrations. We also propose to use this dataset for the task of mapping 3rd person video features to robot trajectories. Furthermore, we present two different approaches using this dataset and evaluate the predicted robot trajectories against ground-truth trajectories. We hope our dataset inspires research in multiple areas including visual imitation, trajectory prediction, and multi-task robotic learning.

==> dump.tex <==
\subsection{Trajectory Generation}

The purpose of this experiment is to evaluate the trajectories we can generate using the sequential joint angle states of the various trajectories. We jointly trained all the different task types. While training either of the systems, at every step the current state of the joint angles was fed in and the state at the next time step was predicted as the output. The key idea behind this was to see given varying lengths of the trajectory sequence what the most likely output trajectory would be.

% \textbf{Model 1: }

\begin{align}
&h_t, c_t = \LSTM(p_t, h_{t-1}, c_{t-1}) \\ 
&y_t = W_2\RELU(W_1h_t + b_1) + b_2
\end{align}


where $p_t$ refers to the token at time step $t$. At test time, $p_t$ is the prediction at the previous time step, $y_{t-1}$. To avoid exposure bias, we train our LSTM by inputting gold token $x_t$ with a probability $p$ and the previous predicted token $y_{t-1}$ with a probability of $1-p$ (We use $p$ = 0.5 in our experiments). $y_t$ is a 14 dimensional vector representing the 14 joint angles of the robot arm.

% \textbf{Model 2: }

In the second model we additionally also pass the token corresponding to the task number as a one hot encoding at the second layer.

\begin{align}
% &h_t, c_t = \LSTM(p_t, h_{t-1}, c_{t-1}) \\ 
&y_t = W_2 concatenated(\RELU(W_1h_t + b_1),t_1) + b_2
\end{align}


 Where $t_1$ is a one hot encoding of the task number.We optimize a regression loss between $y_t$ and the joint angles at the next time step $x_{t+1}$ for each time step to obtain the loss for a data point: 


% \begin{align}
%     \mathcal{L} = \frac{1}{T}\sum_{t=1}^{T}{(x_{t+1} - y_t)^2}
% \end{align}




% This was modelled using an LSTM followed by two neural network layers. The trajectories were subsampled to ensure that they were not too long for the lstm to forget. The input to the network was the time series data of the joint angle trajectories fed in one step at a time. At the training time, at every step when the time series input was required, we selectively used the true state of the joint angles as input with a probability p and with a probability of (1-p) fed in the state predicted at the previous step by the network. This was done to ensure that the conditions that the network saw at train time were close to those that it would see at test time, as at the test time we wanted to be able to pass the predicted joint angle state at every time step of the model to the next step sequentially. 

\textbf{Results: }When jointly trained, the generated trajectory appeared like an average trajectory of the robot hands approaching the table and waiting for sometime before finally moving back to the home position. It couldn't learn any meaningful intricate action, but only learnt to predict an average trajectory. The MSE was 1.0540. The MSE when the LSTM is trained with task labels is 1.0162. This shows that the with the additional information about the task type for every data point, the system learns a better model to predict the task's trajectory.
